Localizing Anomalies in Critical Infrastructure using Model-Based Drift Explanations

Facing climate change, the already limited availability of drinking water will decrease in the future rendering drinking water an increasingly scarce resource. Considerable amounts of it are lost through leakages in water transportation and distribution networks. Thus, anomaly detection and localization, in particular for leakages, are crucial but challenging tasks due to the complex interactions and changing demands in water distribution networks. In this work, we analyze the effects of anomalies on the dynamics of critical infrastructure systems by modeling the networks employing Bayesian networks. We then discuss how the problem is connected to and can be considered through the lens of concept drift. In particular, we argue that model-based explanations of concept drift are a promising tool for localizing anomalies given limited information about the network. The methodology is experimentally evaluated using realistic benchmark scenarios. To showcase that our methodology applies to critical infrastructure more generally, in addition to considering leakages and sensor faults in water systems, we showcase the suitability of the derived technique to localize sensor faults in power systems.

==> src/img/appx/network/tbl.tex <==
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_LogisticRegression} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_LogisticRegression} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_LogisticRegressionSparse} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_LogisticRegressionSparse} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_FeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_FeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_LinearSVM} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_LinearSVM} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_FeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_FeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_PermutationFeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_PermutationFeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_PermutationFeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_PermutationFeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_Mean} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_Mean} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_Random} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_Random} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_FeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_FeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_PermutationFeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_PermutationFeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_FeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_FeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_length_PermutationFeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_best_3_simple_PermutationFeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_LogisticRegression} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_LogisticRegression} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_LogisticRegressionSparse} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_LogisticRegressionSparse} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_FeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_FeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_LinearSVM} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_LinearSVM} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_FeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_FeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_PermutationFeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_PermutationFeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_PermutationFeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_PermutationFeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_Mean} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_Mean} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_Random} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_Random} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_FeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_FeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_PermutationFeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_PermutationFeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_FeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_FeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_length_PermutationFeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_num_closer_simple_PermutationFeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_LogisticRegression} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_LogisticRegression} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_LogisticRegressionSparse} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_LogisticRegressionSparse} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_FeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_FeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_LinearSVM} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_LinearSVM} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_FeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_FeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_PermutationFeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_PermutationFeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_PermutationFeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_PermutationFeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_Mean} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_Mean} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_Random} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_Random} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_FeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_FeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_PermutationFeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_PermutationFeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_FeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_FeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_length_PermutationFeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_rel_dist_simple_PermutationFeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_LogisticRegression} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_LogisticRegression} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_LogisticRegressionSparse} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_LogisticRegressionSparse} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_FeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_FeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_LinearSVM} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_LinearSVM} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_FeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_FeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_PermutationFeatureImportanceET} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_PermutationFeatureImportanceET} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_PermutationFeatureImportance} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_PermutationFeatureImportance} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_Mean} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_Mean} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_Random} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_Random} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_FeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_FeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_PermutationFeatureImportanceRF_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_PermutationFeatureImportanceRF_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_FeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_FeatureImportanceET_wDD} 
\end{tabular}\\
\begin{tabular}{cc}
    \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_length_PermutationFeatureImportanceET_wDD} & \includegraphics[width=0.475\textwidth]{src/img/appx/network/007_found_dist_simple_PermutationFeatureImportanceET_wDD} 
\end{tabular}\\

==> src/tab/results.tex <==
\begin{tabular}
{l@{\:\:}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l}
\toprule
{method} & \multicolumn{3}{l}{\:distance ($-$)} & \multicolumn{3}{l}{\:\numCloser\, ($-$)} & \multicolumn{3}{l}{\:\relDist\, ($-$)} & \multicolumn{3}{l}{\:\bestThree\, ($+$)} \\
& m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$\\
\midrule
Random          &       27 &  29.70 &  16.85 &       14 &  13.94 &  8.36 &     6.5 &  9.47 &  9.76 &    0 &  0.31 &  0.51 \\
Mean            &       17 &  18.97 &  12.83 &        7 &   8.01 &  6.38 &     3.8 &  5.84 &  6.56 &    1 &  0.70 &  0.77 \\
\midrule
FI (RF)         &        5 &   5.09 &   4.04 &        0 &   0.51 &  1.73 &     1.0 &  1.18 &  1.21 &    1 &  1.24 &  0.50 \\
FI (ET)         &        5 &   5.03 &   3.80 &        0 &   0.48 &  1.59 &     1.0 &  1.17 &  1.24 &    2 &  1.81 &  0.63 \\
PFI (RF)        &        5 &   5.03 &   3.50 &        0 &   0.47 &  1.33 &     1.0 &  1.15 &  0.82 &    1 &  1.28 &  0.52 \\
PFI (ET)        &        5 &   5.00 &   3.45 &        0 &   0.46 &  1.34 &     1.0 &  1.16 &  1.10 &    2 &  1.86 &  0.64 \\
SVM             &        5 &   9.72 &  13.67 &        0 &   3.29 &  7.82 &     1.0 &  2.38 &  4.23 &    2 &  1.49 &  0.78 \\
LogR (l2)       &        7 &  14.54 &  14.56 &        1 &   6.30 &  8.59 &     1.2 &  4.02 &  5.55 &    1 &  1.23 &  0.96 \\
LogR (l1)       &        6 &  13.82 &  15.08 &        1 &   5.75 &  8.66 &     1.0 &  3.80 &  5.70 &    1 &  1.18 &  0.88 \\
\midrule
FI (RF w/o DD)  &        5 &  10.18 &  12.97 &        0 &   4.20 &  8.29 &     1.0 &  2.31 &  3.38 &    1 &  0.99 &  0.55 \\
FI (ET w/o DD)  &        5 &   8.04 &  10.55 &        0 &   2.64 &  6.82 &     1.0 &  1.79 &  2.50 &    1 &  1.26 &  0.68 \\
PFI (RF w/o DD) &        5 &   5.99 &   5.79 &        0 &   1.12 &  3.07 &     1.0 &  1.34 &  1.11 &    1 &  1.10 &  0.49 \\
PFI (ET w/o DD) &        5 &  10.94 &  11.23 &        0 &   4.30 &  6.58 &     1.0 &  2.43 &  2.71 &    1 &  0.76 &  0.52 \\
\bottomrule
\end{tabular}

==> src/tab/results_geo.tex <==
\begin{tabular}
{l@{\:\:}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l@{\quad}c@{\:\:}r@{$\pm$}l}
\toprule
{method} & \multicolumn{3}{l}{\:\:distance ($-$)} & \multicolumn{3}{l}{\:\:\numCloser ($-$)} & \multicolumn{3}{l}{\:\:\relDist ($-$)} & \multicolumn{3}{l}{\:\:\bestThree ($+$)} \\
& m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$ & m & $\mu$ & $\sigma$\\
\midrule
Random          &    1206.78 &  1347.67 &  783.45 &       14.0 &  13.96 &  8.36 &     7.53 &  11.76 &  13.60 &    0.0 &  0.31 &  0.51 \\
Mean            &     730.66 &   837.70 &  586.64 &        7.0 &   7.88 &  6.29 &     4.27 &   6.90 &   8.04 &    1.0 &  0.71 &  0.77 \\
\midrule
FI (RF)         &     183.00 &   207.36 &  182.08 &        0.0 &   0.56 &  1.67 &     1.00 &   1.24 &   1.02 &    1.0 &  1.25 &  0.50 \\
FI (ET)         &     180.22 &   204.29 &  170.32 &        0.0 &   0.52 &  1.51 &     1.00 &   1.23 &   0.99 &    2.0 &  1.83 &  0.59 \\
PFI (ET)        &     180.22 &   203.08 &  153.39 &        0.0 &   0.51 &  1.30 &     1.00 &   1.22 &   0.90 &    2.0 &  1.89 &  0.60 \\
PFI (RF)        &     183.00 &   205.33 &  159.14 &        0.0 &   0.53 &  1.35 &     1.00 &   1.23 &   0.92 &    1.0 &  1.30 &  0.52 \\
SVM             &     212.39 &   435.81 &  647.79 &        0.0 &   3.50 &  7.96 &     1.00 &   3.01 &   6.28 &    2.0 &  1.50 &  0.78 \\
LogR (l2)       &     295.26 &   659.34 &  685.25 &        1.0 &   6.53 &  8.69 &     1.31 &   5.07 &   7.91 &    1.0 &  1.23 &  0.97 \\
LogR (l1)       &     268.50 &   627.08 &  711.75 &        1.0 &   5.99 &  8.80 &     1.09 &   4.85 &   8.23 &    1.0 &  1.19 &  0.89 \\
\midrule
FI (RF w/o DD)  &     211.07 &   460.35 &  612.80 &        0.0 &   4.48 &  8.44 &     1.00 &   2.70 &   3.95 &    1.0 &  0.96 &  0.54 \\
FI (ET w/o DD)  &     195.34 &   359.68 &  513.24 &        0.0 &   2.89 &  7.16 &     1.00 &   2.08 &   3.10 &    1.0 &  1.24 &  0.67 \\
PFI (RF w/o DD) &     192.25 &   256.00 &  277.81 &        0.0 &   1.23 &  3.19 &     1.00 &   1.51 &   1.60 &    1.0 &  1.09 &  0.49 \\
PFI (ET w/o DD) &     242.40 &   502.63 &  523.98 &        0.0 &   4.65 &  6.67 &     1.00 &   3.03 &   3.84 &    1.0 &  0.73 &  0.53 \\
\bottomrule
\end{tabular}
